Noisy Heuristics NAS: A Network Morphism based Neural Architecture Search using Heuristics

Network Morphism based Neural Architecture Search (NAS) is one of the most efficient methods, however, knowing where and when to add new neurons or remove dis-functional ones is generally left to black-box Reinforcement Learning models. In this paper, we present a new Network Morphism based NAS called Noisy Heuristics NAS which uses heuristics learned from manually developing neural network models and inspired by biological neuronal dynamics. Firstly, we add new neurons randomly and prune away some to select only the best fitting neurons. Secondly, we control the number of layers in the network using the relationship of hidden units to the number of input-output connections. Our method can increase or decrease the capacity or non-linearity of models online which is specified with a few meta-parameters by the user. Our method generalizes both on toy datasets and on real-world data sets such as MNIST, CIFAR-10, and CIFAR-100. The performance is comparable to the hand-engineered architecture ResNet-18 with the similar parameters.

==> 02_background.tex <==
\section{Background and Related Works}
\label{sec:background}

This section discusses the relevant literature and ideas for Network Morphism based Neural Architecture Search. 

\subsection{Neural Architecture Search (NAS)}

Various methods have been used to conduct NAS. Many of the methods use Reinforcement Learning (RL)\cite{zoph2016neural, baker2016designing} or Genetic Algorithm~\cite{desell2017large} to find network architectures. Such methods train thousands of models and throw away trained models resulting in large computational costs and huge carbon footprint~\cite{strubell2019energy}. A better method would be path selection methods such as DARTS\cite{liu2018darts}. It uses large computation for training and the resultant network is only a subset of the complete network. Such methods are more efficient than RL or Genetic Algorithm based methods.

Network Morphism is another method for efficient architecture search~\cite{cai2018efficient,jin2019auto,elsken2017simple, lu2018compnet, dai2019nest} that aims to search architecture by changing the capacity of the model architecture without changing the learned function. Such systems are constantly changing the number of layers and neurons to better fit the data or accommodate the new data. Network Morphism based NAS also use some other form of models such as Reinforcement Learning~\cite{cai2018efficient} or Bayesian Optimization~\cite{jin2019auto} for morphing the architecture. A variation of this method is pruning based architecture search~\cite{leclerc2018smallify}. Yet this method involves starting with a large network at first which is inefficient.% if final architecture is relatively small. 

MorphNet~\cite{gordon2018morphnet} uses squeezing and expanding of neurons to iteratively regularize flops or throughput of base architecture, however, they do not change the number of layers. Furthermore, network growth through network morphism and compression using pruning for efficiency has been used in incremental learning~\cite{dai2020incremental} and continual learning~\cite{zhang2020regularize}. These methods, used in different settings, resemble with our method of searching new architecture through similar iterative growth and shrink phases. 

\subsection{Network Morphism (Transformation)}

Network Morphism (or Network Transformation) is the process of changing the architecture, the neurons and layers, without changing the function represented by the initial network. After network morphism, networks can be trained further to fit the data better, without requiring to train a new network from scratch.

Network Morphism has mainly two operations: increase the number of layers or the number of neurons. Initial work on Net2Net~\cite{chen2015net2net} showed promising results for increasing the capacity of the model without retraining the whole network. Newer and better methods on increasing the number of neurons and layers has been proposed~\cite{elsken2019neural, wei2016network, wu2019splitting, evci2022gradmax}. We use similar techniques in our method as well.

\subsection{Structured Pruning of Neurons and Layers}

Pruning is widely used to reduce model complexity and to reduce the parameters of the model. Pruning of weights is not generally used for changing the structure of network.Structured pruning, i.e. neuron, filter/channel pruning is generally considered for changing the structure of network. 

There are various methods used for pruning neurons based on magnitude, activation or other metrics~\cite{vadera2020methods}. Efficient method for pruning was explored much earlier in Optimal Brain Damage~\cite{lecun1989optimal} and optimal Brain Surgeon~\cite{hassibi1993optimal}. Newer works have explored neuron significance~\cite{yu2018nisp} or importance~\cite{molchanov2016pruning, molchanov2019importance} based metric derived from the forward and backward signals. Other methods prune group of neurons or even layers or paths using group lasso regularization~\cite{friedman2010note, wen2016learning}. Our method uses pruning to guide the search process by correcting for the noisy addition of new neurons.


% Neuron pruning and layer pruning has been used widely in Network Morphism based NAS. ... uses Neuron pruning along with Neuron addition for incremental learning and .. uses it for neural architecture search.

% Our method differs from the above methods in following aspects. We make heuristics based method learned from manually developing the architectures. These methods use it alongside RL based method to make compact network. In our method, adding and pruning is fundamental to the Noisy Search Mechanism which guides the growth or decay of the network. 







